Constrained Correlated Equilibria

This paper introduces constrained correlated equilibrium, a solution concept combining correlation and coupled constraints in finite non-cooperative games. In the general case of an arbitrary correlation device and coupled constraints in the extended game, we study the conditions for equilibrium. In the particular case of constraints induced by a feasible set of probability distributions over action profiles, we first show that canonical correlation devices are sufficient to characterize the set of constrained correlated equilibrium distributions and provide conditions of their existence. Second, it is shown that constrained correlated equilibria of the mixed extension of the game do not lead to additional equilibrium distributions. Third, we show that the constrained correlated equilibrium distributions may not belong to the polytope of correlated equilibrium distributions. Finally, we illustrate these results through numerical examples.

==> sections/Appendices/GNE_Equivalent_Definition.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{proposition}\label{prop:AlternativeGNEDefinition}
Let $G = (\mathcal{N}, (\mathcal{S}_i)_{i\in\mathcal{N}}, {(u_i)}_{i\in\mathcal{N}})$ be non-cooperative game, $\mathcal{R} \subseteq \mathcal{X}$ a feasible set of strategy profiles 
%and for any $\bm{x}_{-i} \in \mathcal{S}_{-i}$ $\mathcal{K}_i(\bm{x}_{-i}) = \{ x_i \in \mathcal{S}_{i} : (x_i, \bm{x}_{-i}) \in \mathcal{R} \}$ the constraint correspondence for player $i$. 
The strategy profile $\bm{x}^* \in \mathcal{S}$ is a generalized Nash equilibrium of $G$ 
if and only if
$\bm{x}^{*} \in \mathcal{R}$ 
and
for any $i\in\mathcal{N}$, 
for any $x^\prime_i \in \mathcal{K}_i(\bm{x}_{-i}^{*})$, 
%%%%%%%%%%%%%%%%%%
    \begin{equation} 
        u_i(x^*_i, \bm{x}_{-i}^{*}) \geq u_i(x^\prime_i,\bm{x}_{i}^{*})
    \end{equation}
    %%%%%%%%%%%%%%%%%%
\end{proposition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{proof} 
    Let $\bm{x}^*$ be a generalized Nash equilibrium. 
    By definition, we have,
    %%%%%%%%%%%%%%%%%%
    \begin{align}
            \forall i \in \mathcal{N}, 
            x_i^* \in \underset{x_i \in \mathcal{K}_i(\bm{x}_{-i}^{*})}{\arg \max } u_i(x_i, \bm{x}_{-i}^{*}) \nonumber
    \end{align}
    %%%%%%%%%%%%%%%%%%
    furthermore,  
    \begin{equation}
        \underset{x_i \in \mathcal{K}_i(\bm{x}_{-i}^{*})}{\arg \max } u_i(x_i, \bm{x}_{-i}^{*}) 
        =
        \{
            x_i \in \mathcal{K}_i(\bm{x}_{-i}^{*}) 
            \mid 
            \forall x^\prime_i \in \mathcal{K}_i(\bm{x}_{-i}^{*}), 
            u_i(x_i, \bm{x}_{-i}^{*}) \geq u_i(x^\prime_i, \bm{x}_{-i}^{*})
        \} \nonumber
    \end{equation}
    then, $\bm{x}^*$ is a generalized Nash equilibrium 
    if and only if,
    \begin{equation}
        \forall i\in\mathcal{N},
        x_i^* 
        \in 
        \{
            x_i \in \mathcal{K}_i(\bm{x}_{-i}^{*}) 
            \mid 
            \forall x^\prime_i \in \mathcal{K}_i(\bm{x}_{-i}^{*}), 
            u_i(x_i, \bm{x}_{-i}^{*}) \geq u_i(x^\prime_i, \bm{x}_{-i}^{*})
        \}
    \end{equation}
    The latter formula is equivalent to, 
    %%%%%%%%%%%%%%%%%%
    \begin{equation}\label{eq:GNE_Equivalent}
        \forall i\in\mathcal{N},
        \left(
            \bm{x}_i^{*} \in \mathcal{K}_i(\bm{x}_{-i}^{*})
            \wedge 
            \left(
            \forall x^\prime_i \in \mathcal{K}_i(\bm{x}_{-i}^{*}), 
            u_i(x^*_i, \bm{x}_{-i}^{*}) \geq u_i(x^\prime_i, \bm{x}_{-i}^{*})
            \right)
        \right)
    \end{equation}
    %%%%%%%%%%%%%%%%%%
    
    %\st{Using the distributive property of the quantifier,} \eqref{eq:GNE_Equivalent} is written
    %===================
    %$\Leftrightarrow$ (Distributivity of $ \forall i\in\mathcal{N}$ TBC)
    %===================
    which is equivalent to,
    %%%%%%%%%%%%%%%%%%
    \begin{equation}
        \left(
        \forall i \in \mathcal{N},
        \bm{x}_i^{*} \in \mathcal{K}_i(\bm{x}_{-i}^{*})
        \right)
        \wedge
        \left(
            \forall i \in \mathcal{N},
            \forall x^\prime_i \in \mathcal{K}_i(\bm{x}_{-i}^{*}), 
            u_i(x^*_i, \bm{x}_{-i}^{*}) \geq u_i(x^\prime_i, \bm{x}_{-i}^{*})
        \right)
    \end{equation}
    %%%%%%%%%%%%%%%%%%
    Furthermore, 
    $
        \left( \forall i\in\mathcal{N}, x_i^*\in \mathcal{K}_i(\bm{x}_{-i}^*)\right) \Leftrightarrow \bm{x}^*\in\mathcal{R}
    $.
    Then, the latter formula is equivalent to,
    %===================
    %%%%%%%%%%%%%%%%%%
    \begin{equation} 
        \bm{x}^{*} \in \mathcal{R}
        \wedge
        \left(
            \forall i \in \mathcal{N},
            \forall x^\prime_i \in \mathcal{K}_i(\bm{x}_{-i}^{*}), 
            u_i(x^*_i, \bm{x}_{-i}^{*}) \geq u_i(x^\prime_i, \bm{x}_{-i}^{*})
        \right) \nonumber
    \end{equation}
    Thus, $\bm{x}^*$ is a generalized Nash equilibrium if and only if $\bm{x}^* \in \mathcal{R}$ and 
    for any $i\in\mathcal{N}$, 
    for any $x^\prime_i \in \mathcal{K}_i(\bm{x}_{-i}^{*})$, 
    %%%%%%%%%%%%%%%%%%
    \begin{equation} 
        u_i(x^*_i, \bm{x}_{-i}^{*}) \geq u_i(x^\prime_i,\bm{x}_{-i}^{*})
    \end{equation}
    %%%%%%%%%%%%%%%%%%    
    %%%%%%%%%%%%%%%%%%
    % Lastly,
    % \textcolor{red}{
    %     %%%%%%%%%%%%%%%%%%
    %     \begin{equation} 
    %         \bm{x}^{*} \in \mathcal{R}
    %         \text{ and }
    %             \forall i \in \mathcal{N},
    %             \forall x_i \in \mathcal{K}_i(\bm{x}_{-i}^{*}), 
    %             u_i(x^*_i, \bm{x}_{-i}^{*}) \geq u_i(x_i, \bm{x}_{i}^{*}) \nonumber
    %     \end{equation}
    %     %%%%%%%%%%%%%%%%%%
    % }
    Furthermore, for any $i\in\mathcal{N}$, ${x}^\prime_{i} \in \mathcal{K}_{i}(\bm{x}^*_{-i})$ if and only if $(x^\prime_i, \bm{x}^*_{-i}) \in \mathcal{R}$. Hence,  $\bm{x}^*$ is a generalized Nash equilibrium if and only if $\bm{x}^* \in \mathcal{R}$ and for any $i\in\mathcal{N}$, 
    for any $x^\prime_i \in \mathcal{S}_{i}$ such that $(x^\prime_i, \bm{x}^*_{-i}) \in \mathcal{R}$, 
    \begin{equation} 
        u_i(x^*_i, \bm{x}_{-i}^{*}) \geq u_i(x^\prime_i,\bm{x}_{-i}^{*})
    \end{equation}
    \begin{flushright}
    $\blacksquare$
    \end{flushright}
\end{proof} 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> sections/Appendices/Preliminaries.tex <==
\begin{proposition}
        Let $G$ be a finite non-cooperative game and $d= (\Omega, (\mathcal{P}_i)_{i\in\mathcal{N}}, \bm{q})$ a correlation device. The strategy $\bm{\alpha}^* = (\alpha_i^*)_{i \in \mathcal{N}} : \Omega \rightarrow \mathcal{A}$ is a correlated equilibrium if and only if
    \begin{equation}
        \sum_{\omega \in \Omega} \bm{q}(\omega) \left[u_{i}({\alpha}_i^*(\omega), \bm{\alpha}_{-i}^*(\omega)) - u_{i}(\tau^\prime_i(\omega), \bm{\alpha}^*_{-i}(\omega))\right] \geq 0
    \end{equation}
    for every player $i$ and every $\tau_i^\prime$ function of $\alpha^*_i$.
\end{proposition}
%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{proof}
Suppose $\bm{\alpha}^*= (\alpha^*_i)_{i \in \mathcal{N}}$ is an $n$-tuple of correlated strategies with $\alpha_i^* : \Omega \rightarrow \mathcal{A}_i$ satisfying
%%%%%%%%%%%%%%%%%%%
\begin{align}
    \sum_{\omega \in \Omega} \bm{q}(\omega) \left[u_{i}({\alpha}_i^*(\omega),\bm{\alpha}_{-i}^*(\omega)) - u_{i}(\tau^\prime_i(\omega), \bm{\alpha}^*_{-i}(\omega))\right] \geq 0 \label{eq:defn1}
\end{align}
%%%%%%%%%%%%%%%%%%%
for each player $i$ and each $\tau^\prime_i$ function of $\alpha_i^*$. The function $\tau_i^\prime$ that are function of $\alpha_i^*$ are in the set:
%%%%%%%%%%%%%%%%%%%
\begin{align}
    \Theta_{\alpha_i^*} = \{ \alpha^\prime_i : \Omega \rightarrow \mathcal{A}_i \text{ s.t } \exists h_i : {\mathcal{A}_i} \rightarrow {\mathcal{A}_i} \mid  \alpha^\prime_i = h_i \circ \alpha_i^* \}
\end{align}
%%%%%%%%%%%%%%%%%%%
Hence, we can re-write the conditions in Eq. (\ref{eq:defn1}) satisfied by $\bm{\alpha}^*$ as follows:
%%%%%%%%%%%%%%%%%%%
\begin{align}
    \forall i \in \mathcal{N},
    \forall \tau_i^\prime \in \Theta_{\alpha^*_i} 
    \quad
    \sum_{\omega \in \Omega} \bm{q}(\omega) \left[u_{i}({\alpha}_i^*(\omega),\bm{\alpha}_{-i}^*(\omega)) - u_{i}(\tau^\prime_i(\omega), \bm{\alpha}^*_{-i}(\omega))\right] \geq 0
\end{align}
%%%%%%%%%%%%%%%%%%%
\noindent Now, consider the correlation device $d = (\Omega, (\mathcal{P}_i)_{i \in \mathcal{N}}, \bm{q})$ where the partition $\mathcal{P}_i$ is induced by player $i$'s equilibrium strategy $\alpha_i^*$:
%%%%%%%%%%%%%%%%%%%
\begin{align}
    \mathcal{P}_i = \{ \omega \in \Omega : \alpha_i^{*}(\omega) = a_i \}_{a_i \in \mathcal{A}_i}
\end{align}
%%%%%%%%%%%%%%%%%%%
We prove that the strategies $\tau_i^\prime$ in the set $\Theta_{{\alpha}^*_i}$ are exactly the $\mathcal{P}_i$-measurable mappings $\alpha_i^* : \Omega \rightarrow \mathcal{A}_i$ in $\mathcal{S}_{i, d}$ \ie $\mathcal{S}_{i,d} = \Theta_{\bm{\alpha}^*_i}$ for every player $i$.\\
%\textcolor{red}{Consider the $\sigma$-algebra generated by the partition $\mathcal{P}_i$ denoted by $\sigma(\mathcal{P}_i)$ consisting of all possible unions of the elements of the partition (including the empty set).}\\
By definition, the function $\tau^\prime_i: \Omega \rightarrow \mathcal{A}_i$ is measurable with respect to the $\sigma$-algebra $\sigma(\mathcal{P}_i)$ generated by the partition $\mathcal{P}_i$ if and only if $\tau_i^{\prime}$ is constant on each set element of the partition.\\
Let $P_{a_i} \in \mathcal{P}_i$ be the element of the partition such that $\forall \omega \in P_{a_i}, \alpha_i^*(\omega) = a_i$ , we have:
%%%%%%%%%%%%%%%%%%%
\begin{align}
    \forall \omega \in P_{a_i},
    \quad \tau_i^{\prime}(\omega) & = (h_i \circ \alpha_i^*)(\omega) = h_i ( \alpha_i^*(\omega)) = h_i(a_i)
\end{align}
%%%%%%%%%%%%%%%%%%%
Hence the function is constant on the element of the partition $P_{a_i}$. Therefore, the function $\tau_i^\prime$ are the $\mathcal{P}_i$-measurable functions and $\Theta_{{\alpha}^*_i} = \mathcal{S}_{i, d}$.
To conclude, the two definitions are equivalent and characterize the same set of $n$-tuples of correlated equilibrium strategies.
\begin{flushright}                                      
$\blacksquare$
\end{flushright}
\end{proof}


%\section*{Appendix B}
\newpage

\begin{proposition}
    Let $G$ be a finite non-cooperative game and $d= (\Omega, (\mathcal{P}_i)_{i\in\mathcal{N}}, \bm{q})$ a correlation device. The strategy $\bm{\alpha}^* = (\alpha_i^*)_{i \in \mathcal{N}} : \Omega \rightarrow \mathcal{A}$ is a correlated equilibrium if and only if
    \begin{align}
        & \forall i \in \mathcal{N},
        \forall a_{i} \in \mathcal{A}_{i},
        \forall \omega \in \Omega \nonumber \\
        & \sum_{\omega^{\prime} \in P_{i}(\omega)} \bm{q}(\omega^{\prime}) \left[u_{i}({\alpha}_i^*(\omega^{\prime}), \bm{\alpha}_{-i}^*(\omega^{\prime})) - u_{i}(a_i, \bm{\alpha}^*_{-i}(\omega^{\prime}))\right] \geq 0 
    \end{align}
\end{proposition}

\begin{proof}
$(\Rightarrow)$
We suppose that $\bm{\alpha}^*$ is a correlated equilibrium strategy satisfying
\begin{align}
& \forall i \in \mathcal{N},
\forall \alpha^\prime_{i} : \Omega \rightarrow \mathcal{A}_{i} \nonumber\\
& \sum\limits_{\omega^\prime \in \Omega} \bm{q}(\omega^\prime ) u_{i}({\alpha}_i^*(\omega^{\prime}),\bm{\alpha}_{-i}^*(\omega^\prime)) \geq \sum\limits_{\omega^\prime \in \Omega} \bm{q}(\omega^\prime) u_{i}(\alpha^\prime_{i}(\omega^\prime), \bm{\alpha}^*_{-i}(\omega^\prime)) \label{eq:average}
\end{align}
Let $\mathcal{P}_i = \{  P_{i, 1}, P_{i, 2}, ..., P_{i, n_i} \}$ and consider the deviation strategy $\alpha^\prime_i$ in Eq. (\ref{eq:strategy}), equal to player $i$'s equilibrium strategy $\alpha_i^*$ except on a single element of the partition
\begin{align}\label{eq:strategy}
    \alpha^\prime_i(\omega^\prime) = 
    \begin{cases}
    \alpha^*_i(\omega^\prime), & \text { if } \omega^\prime \in \Omega - \{P_{i, j}\}, \\
    a_i, & \text { otherwise. }
    \end{cases}
\end{align}
Eq. (\ref{eq:average}) can be written for any player $i \in \mathcal{N}$ and any strategy $\alpha^\prime_i$ of the form Eq. (\ref{eq:strategy})
\begin{align}
    \sum\limits_{\mathclap{\omega^\prime \in P_{i, j}}} \bm{q}(\omega^\prime ) u_{i}({\alpha}_i^*(\omega^{\prime}), \bm{\alpha}_{-i}^*(\omega^\prime)) + \sum\limits_{\mathclap{\omega^\prime \in \Omega - \{P_{i, j}\}}} \bm{q}(\omega^\prime ) u_{i}({\alpha}_i^*(\omega^{\prime}),\bm{\alpha}_{-i}^*(\omega^\prime)) \geq \nonumber \\
    \sum\limits_{\mathclap{\omega^\prime \in P_{i, j}}} \bm{q}(\omega^\prime) u_{i}(a_{i}, \bm{\alpha}^*_{-i}(\omega^\prime)) + \sum\limits_{\mathclap{\omega^\prime \in \Omega - \{P_{i, j}\}}} \bm{q}(\omega^\prime) u_{i}(\alpha_{i}^*(\omega^\prime), \bm{\alpha}^*_{-i}(\omega^\prime))
\end{align}
Hence, after simplifying the second term on both sides, we obtain
\begin{align}
    \sum\limits_{\omega^\prime \in P_{i, j}} \bm{q}(\omega^\prime ) u_{i}({\alpha}_i^*(\omega^{\prime}),\bm{\alpha}_{-i}^*(\omega^\prime)) \geq \sum\limits_{\omega^\prime \in P_{i, j}} \bm{q}(\omega^\prime) u_{i}(a_{i}, \bm{\alpha}^*_{-i}(\omega^\prime))
\end{align}
Let $\omega \in P_{i,j}$, and denote the partition the j$^{th}$ element of player $i$'s partitioning $P_{i,j}$ containing $\omega$ by $P_{i,j}= P_i(\omega)$.
We then have
\begin{align}
    & \forall i \in \mathcal{N},
    \forall a_{i} \in \mathcal{A}_i,
    \forall \omega \in \Omega \nonumber \\
    & \sum\limits_{\omega^\prime \in P_{i}(\omega)} \bm{q}(\omega^\prime ) u_{i}({\alpha}_i^*(\omega^{\prime}),\bm{\alpha}_{-i}^*(\omega^\prime)) \geq \sum\limits_{\omega^\prime \in P_{i}(\omega)} \bm{q}(\omega^\prime) u_{i}(a_{i}, \bm{\alpha}^*_{-i}(\omega^\prime))
\end{align}
$(\Leftarrow)$ We now assume that the strategy $\bm{\alpha}^*$ satisfies,
\begin{align}
    & \forall i \in \mathcal{N},
    \forall a_i \in \mathcal{A}_{i},
    \forall \omega \in \Omega \nonumber \\
    & \sum_{\omega^{\prime} \in P_{i}(\omega)} \bm{q}(\omega^{\prime}) u_{i}({\alpha}_i^*(\omega^{\prime}),\bm{\alpha}_{-i}^*(\omega^{\prime})) \geq \sum_{\omega^{\prime} \in P_{i}(\omega)} \bm{q}(\omega^{\prime}) u_{i}(a_{i}, \bm{\alpha}^*_{-i}(\omega^{\prime})) \label{eq:conditionalInequality}
\end{align}
Let $\mathcal{P}_i = \{  P_{i, 1}, P_{i, 2}, ..., P_{i, n_i} \}$.
The inequalities in Eq. (\ref{eq:conditionalInequality}) imply
\begin{align}
    & \forall i \in \mathcal{N},
    \forall a_{i} \in \mathcal{A}_i,
    \forall P_{i,j} \in \mathcal{P}_i \nonumber \\
    & \sum_{\omega^{\prime} \in P_{i,j}} \bm{q}(\omega^{\prime}) u_{i}({\alpha}_i^*(\omega^{\prime}),\bm{\alpha}_{-i}^*(\omega^{\prime})) \geq \sum_{\omega^{\prime} \in P_{i,j}} \bm{q}(\omega^{\prime}) u_{i}(a_{i}, \bm{\alpha}^*_{-i}(\omega^{\prime}))
\end{align}
Summing over all elements $P_{i,j}$ of the partition $\mathcal{P}_i$,
\begin{align}
    & \forall i \in \mathcal{N},
    \forall \alpha^\prime_{i} : \mathcal{P}_i \rightarrow \mathcal{A}_{i} \\
    & \sum_{ P_{i,j} \in \mathcal{P}_i} \sum_{\omega^{\prime} \in P_{i,j}} \bm{q}(\omega^{\prime}) u_{i}({\alpha}_i^*(\omega^{\prime}),\bm{\alpha}_{-i}^*(\omega^{\prime})) \geq \sum_{P_{i,j} \in \mathcal{P}_i} \sum_{\omega^{\prime} \in P_{i,j}} \bm{q}(\omega^{\prime}) u_{i}(\alpha^\prime_{i}(\omega^\prime), \bm{\alpha}^*_{-i}(\omega^{\prime})) \label{eq:ref} \nonumber
\end{align}
where $\alpha^\prime_i$ is a function mapping each element $P_{i,j}$ of $\mathcal{P}_i$ to an action $a_i \in \mathcal{A}_i$.
Since for every player the set $\mathcal{P}_i$ is a partition of $\Omega$, Eq. (\ref{eq:ref}) is equivalent to
\begin{align}
    & \forall i \in \mathcal{N},
    \forall \alpha^\prime_{i} : \Omega \rightarrow \mathcal{A}_{i} \nonumber \\
    & \sum_{\omega \in \Omega} \bm{q}(\omega) u_{i}({\alpha}_i^*(\omega),\bm{\alpha}_{-i}^*(\omega)) \geq \sum_{\omega \in \Omega} \bm{q}(\omega) u_{i}(\alpha^\prime_{i}(\omega), \bm{\alpha}^*_{-i}(\omega))
\end{align}
\begin{flushright}                                      
$\blacksquare$
\end{flushright}
\end{proof}



\newpage

\begin{proposition}
    Let $G$ be a finite non-cooperative game. The distribution $\bm{p}\in\Delta(\mathcal{A})$ is a correlated equilibrium distribution if and only if
    %%%%%%%%%%%%%%%%%%%
    \begin{align}
        & \forall i \in \mathcal{N},
        \forall \beta_i : \mathcal{A}_i \rightarrow \mathcal{A}_i
        \quad
        \sum\limits_{\bm{a} \in \mathcal{A}} \bm{p}(\bm{a}) \left[u_{i}(a_i, \bm{a}_{-i}) - u_{i}(\beta_i(a_i), \bm{a}_{-i}) \right] \geq 0
    \end{align}
    %%%%%%%%%%%%%%%%%%%
\end{proposition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{proof}
In this proof, we start by showing (by logical equivalence) the $(\Rightarrow)$ implication of the proposition. We show it by contradiction, \ie if
        %%%%%%%%%%%%%%%%%%%
        \begin{align}
            \exists i \in \mathcal{N},
            \exists \beta^\prime_i : \mathcal{A}_i \rightarrow {\mathcal{A}_i}
            \quad \sum\limits_{\bm{a} \in \mathcal{A}} \bm{p}(\bm{a})
            \left[
                u_{i}(a_i, \bm{a}_{-i}) - u_{i}(\beta_i^\prime(a_i), \bm{a}_{-i}) 
            \right] 
            < 0 
        \end{align}
        %%%%%%%%%%%%%%%%%%%
    then, $\bm{p}$ is not a correlated equilibrium distribution.
    %%%%%%%%%%%%%%%%%%%
    Assume that $\bm{p}$ is a correlated equilibrium distribution and let ${\beta}_i^\prime$ such that 
    %%%%%%%%%%%%%%%%%%%
    \begin{equation}
          \nonumber \\
        \quad \sum\limits_{\bm{a} \in \mathcal{A}} \bm{p}(\bm{a})
        \left[
            u_{i}(a_i, \bm{a}_{-i}) - u_{i}({\beta}^\prime_i(a_i), \bm{a}_{-i}) 
        \right] 
        < 0 
    \end{equation}
    %%%%%%%%%%%%%%%%%%%
    Consider the partitioning $\mathcal{P}_i = \{ P_{b_i}\}_{b_i \in \mathcal{A}_i}$ where $P_{b_i} = \{ \omega \in \Omega : \alpha_i^*(\omega) = b_i \}$ for every $i$. We have,
        \begin{align}
            \forall \bm{a} \in \mathcal{A} \quad \bm{p}_{(x_i,\bm{\alpha}_{-i}^*)}(\bm{a}) = 
            p_{(\beta^\prime_i\circ\alpha_i^*,\bm{\alpha}_{-i}^*)}(\bm{a}) = 
              \bm{z}_{\beta^\prime_i, \bm{p}} (\bm{a})
        \end{align}
    %%%%%%%%%%%%%%%%%%%
    Furthermore, we have,
    %%%%%%%%%%%%%%%%%%%
    \begin{align}
        &
        \sum_{\omega\in\Omega} \bm{q}(\omega) 
        \left[
            u_i(\alpha_i^*(\omega),\bm{\alpha}_{-i}^*) 
            -
            u_i(x_i(\omega),\bm{\alpha}_{-i}^*)
        \right]
        \\
        &= 
        \sum_{\bm{a}\in\mathcal{A}}\bm{p}_{\bm{\alpha}^*}(\bm{a})
        \left[
            u_i(a_i,\bm{a}_{-i}) 
            -
            u_i(\beta^\prime_i(a_i),\bm{a}_{-i})
        \right]\\
        &= 
        \sum_{\bm{a}\in\mathcal{A}}\bm{p}(\bm{a})
        \left[
            u_i(a_i,\bm{a}_{-i}) 
            -
            u_i(\beta^\prime_i(a_i),\bm{a}_{-i})
        \right]
        <0
    \end{align}
    %%%%%%%%%%%%%%%%%%%
    where the last equality follows from the definition of $\bm{p}$ and the inequality is from the assumption on $\beta^\prime_i$.
    Then $\bm{\alpha}^*$ is not a correlated equilibrium implying that $\bm{p}$ is not a correlated equilibrium distribution.\\
    %%%%%%%%%%%%%%%%%%%
    ($\Rightarrow$) Let $\bm{p}$ be a probability distribution such that
    %%%%%%%%%%%%%%%%%%%
    \begin{align}
            \forall i \in \mathcal{N},
            \forall \beta_i : \mathcal{A}_i \rightarrow \mathcal{A}_i \quad 
            \sum\limits_{\bm{a} \in \mathcal{A}} \bm{p}(\bm{a}) 
            \left[u_{i}(a_i, \bm{a}_{-i}) - u_{i}(\beta_i(a_i), \bm{a}_{-i}) \right] \geq 0 
            \label{eq}
    \end{align}
    %%%%%%%%%%%%%%%%%%%
Consider the canonical representation with $d=(\mathcal{A},(\mathcal{P}_i)_{i\in\mathcal{N}},\bm{p})$ such that
$\mathcal{P}_i = \{  P_{a_i} \}_{a_i \in \mathcal{A}_i}$. Let now assume  that each player  uses the strategy $\alpha_i^*:\mathcal{A} \rightarrow  \mathcal{A}_i$ such that $\alpha_i^*(\bm{a})=a_i$ $\forall \bm{a} \in P_{a_i}$. Then the relation (\ref{eq}) becomes:
    %%%%%%%%%%%%%%%%%%%
    \begin{align}
        &\forall i \in \mathcal{N}, 
        \forall \beta_i :  \mathcal{A}_i \rightarrow \mathcal{A}_i \nonumber \\
        & \sum\limits_{a_i \in \mathcal{A}_i} \sum\limits_{\omega \in P_{a_i}} \bm{p}(\omega) 
        \left[
            u_{i}(\alpha^*_i(\omega), \bm{\alpha}^*_{-i}(\omega)) - u_{i}(\beta_i(a_i), \bm{\alpha}^*_{-i}(\omega)) 
        \right] 
        \geq 0
    \end{align}
    %%%%%%%%%%%%%%%%%%%
Let define $\alpha_i^\prime : \mathcal{A} \rightarrow \mathcal{A}_i$ the deviation of player $i$. This means that the player $i$ makes a deviation on different partitions from $\alpha^*_i$. Therefore, any deviation  $\alpha_i^\prime$ can be expressed in terms of this deviation as follows:  $\alpha^\prime_i = \beta_i\circ \alpha^*_i$, where $\beta_i$ is a mapping from $\mathcal{A}_i \rightarrow \mathcal{A}_i$. We have 
\begin{align}
            & \sum\limits_{a_i \in \mathcal{A}_i} \sum\limits_{\omega \in P_{a_i}} \bm{p}(\omega) 
        \left[
            u_{i}(\alpha^*_i(\omega), \bm{\alpha}^*_{-i}(\omega)) - u_{i}(\alpha_i^\prime(w), \bm{\alpha}^*_{-i}(\omega)) 
        \right] \nonumber\\
    & =
  \sum\limits_{a_i \in \mathcal{A}_i} \sum\limits_{\omega \in P_{a_i}} \bm{p}(\omega) 
        \left[
            u_{i}(\alpha^*_i(\omega), \bm{\alpha}^*_{-i}(\omega)) - u_{i}(\beta_i\circ \alpha^*_i(w), \bm{\alpha}^*_{-i}(\omega)) 
        \right] \nonumber\\  
&=  \sum\limits_{\omega \in \Omega} \bm{q}(\omega) 
        \left[
            u_{i}(\alpha^*_i(\omega), \bm{\alpha}^*_{-i}(\omega)) - u_{i}(\beta(a_i), \bm{\alpha}^*_{-i}(\omega)) 
        \right] \geq 0
         \end{align}
Then $\bm{\alpha}^*$ is a correlated equilibrium strategy and the probability distribution it induces $\bm{p}$ is a correlated equilibrium probability distribution.
\begin{flushright}
$\blacksquare$
\end{flushright}
\end{proof}



==> sections/Appendices/ToBeDiscussed.tex <==
%\begin{enumerate}
    %\item \blue{\st{Quantificateurs dans les phrases ou pas ?}} \textcolor{red}{Quantificateurs dans les phrases enlevés}
    %\item \blue{Où est le resultat qui dit que les devices canoniques ne sont plus suffisants dans le cas generique ?} \textcolor{red}{Ajouter le résultat sous forme de remarque dans la Section 4. Trouver l'endroit adéquat pour le mettre.}\\
    %Juste après la définition.
    % \item \textcolor{red}{Proposition \ref{prop:SmallerConstraints} sur la relation entre les distributions contraintes de deux ensembles à discuter}
    %\item \textcolor{red}{Partie explicant les symboles utilisés à remettre?}
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    %\item \blue{
    %What about the definition of GNE below where the coupled constraint set $\mathcal{R}$ is used explicitly 
    %%%%%%%%%%%%%%%%%%
    %\begin{definition}[Generalized Nash equilibrium]\label{defn:GNE1}
    %    A generalized Nash equilibrium of a generalized game $G'$ is a strategy profile $\bm{x}^{*}\in\mathcal{R}$ such that, 
    %    \begin{align}
    %        \forall i \in \mathcal{N}, 
    %        \forall x_i \in \mathcal{K}_{i,d}(\bm{x}_{-i}^{*}), 
    %        \quad 
    %        u_i(x^*_i, \bm{x}_{-i}^{*}) \geq u_i(x_i, \bm{x}_{-i}^{*}).
    %    \end{align}
    %\end{definition}}
    %%%%%%%%%%%%%%%%%%
    -%\item \blue{An alternative definition of constrained correlated equilibria can be given without references to generalized Nash equilibria.}
        %%%%%%%%%%%%%%%%%%%%%%%
        %\item
        %\textcolor{red}{Tester avec cette définition alternative et comparer les deux. Proposition à prouver et intégrer avec la définition.}
    %%%%%%%%%%%%%%%%%%%%%%%%%
    %\item 
        %\blue{Candidate generalization that would make the previous proposition a corollary and could be used to interpret numerical experiments - from discussion with Rachid 28/03/2023.}

        %%%%%%%%%%%%%%%%%%%    
    % \item \blue{A intégrer ? En quoi n'est-ce pas une conséquence de la Proposition \ref{prop:robustnessToRestrictions} ?} 
    % \textcolor{brown}{
    % %%%%%%%%%%%%%%%%%%%%
    % \begin{proposition}\label{prop:inclusion}
    %     Let $\mathcal{C}$ and $\mathcal{C}^\prime$ be feasible sets of probability distributions such that $\mathcal{C} \subseteq \mathcal{C}^\prime$.
    %     If $\bm{p}^*$ is a constrained correlated equilibrium distribution with respect to $\mathcal{C}$ 
    %     then $\bm{p}^*$ is a constrained correlated equilibrium distribution with respect to $\mathcal{C}^\prime$.
    % \end{proposition}
    % %%%%%%%%%%%%%%%%%%%%
    % %%%%%%%%%%%%%%%%%%%%
    % \begin{proof} 
    %     Let $\mathcal{C}$ and $\mathcal{C}^\prime$ be feasible sets of probability distributions such that $\mathcal{C} \subseteq \mathcal{C}^\prime$. Consider a constrained correlated equilibrium distribution $\bm{p}^*$ with respect to $\mathcal{C}$. By definition, $\bm{p}^* \in \mathcal{C}$ and
    %     $\forall i \in \mathcal{N}, \forall \alpha_i \in {\mathcal{A}_i}^{\mathcal{A}_i} \text{ s.t } {\bm{z}_{\alpha_i, \bm{p}^*}} \in \mathcal{C}$
    %     %%%%%%%%%%%%%%%%%%%
    %     \begin{align}
    %         & \sum_{\bm{a} \in \mathcal{A}} \bm{p}^*(\bm{a})[u_i(\bm{a}) - u_i(\alpha_i(a_i), \bm{a}_{-i})] \geq 0
    %     \end{align}
    %     %%%%%%%%%%%%%%%%%%%
    %     Since $\mathcal{C}^\prime \subseteq \mathcal{C}$, we have the inclusion
    %     %%%%%%%%%%%%%%%%%%%
    %     \begin{align}
    %          \{ \alpha_i \in {\mathcal{A}_i}^{\mathcal{A}_i} : {\bm{z}_{\alpha_i, \bm{p}^*}} \in \mathcal{C}^\prime \}  \subseteq   \{  {\alpha_i \in \mathcal{A}_i}^{\mathcal{A}_i} : {\bm{z}_{\alpha_i, \bm{p}^*}} \in \mathcal{C} \}
    %     \end{align}
    %     %%%%%%%%%%%%%%%%%%%
    %     which implies 
    %     %%%%%%%%%%%%%%%%%%%
    %     \begin{align}
    %         \forall i \in \mathcal{N}, \forall \alpha_i \in {\mathcal{A}_i}^{\mathcal{A}_i} \text{ s.t } {\bm{z}_{\alpha_i, \bm{p}^*}} \in \mathcal{C}^\prime \, \sum_{\bm{a} \in \mathcal{A}} \bm{p}^*(\bm{a})[u_i(\bm{a}) - u_i(\alpha_i(a_i), \bm{a}_{-i})] \geq 0
    %     \end{align}
    %     %%%%%%%%%%%%%%%%%%%
    %     Thus, $\bm{p}^*$ is a constrained correlated equilibrium distribution with respect to $\mathcal{C}^\prime$.
    %     %%%%%%%%%%%%%%%%%%%
    %     \begin{flushright}        
    %     $\blacksquare$
    %     \end{flushright}
    % \end{proof}
    % %%%%%%%%%%%%%%%%%%%
    % }
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\end{enumerate}
